HoloNets: Spectral Convolutions do extend to Directed Graphs

Within the graph learning community, conventional wisdom dictates that spectral convolutional networks may only be deployed on undirected graphs: Only there could the existence of a well-defined graph Fourier transform be guaranteed, so that information may be translated between spatial- and spectral domains. Here we show this traditional reliance on the graph Fourier transform to be superfluous and -- making use of certain advanced tools from complex analysis and spectral theory -- extend spectral convolutions to directed graphs. We provide a frequency-response interpretation of newly developed filters, investigate the influence of the basis used to express filters and discuss the interplay with characteristic operators on which networks are based. In order to thoroughly test the developed theory, we conduct experiments in real world settings, showcasing that directed spectral convolutional networks provide new state of the art results for heterophilic node classification on many datasets and -- as opposed to baselines -- may be rendered stable to resolution-scale varying topological perturbations.

==> Comments <==
Why not tested in homophilic setting?


We provide details ( shed light) on transferability; as this so far has only been considered on undirected graphs. We also on transferability... and [but; ICLR 2023 paper; but not actually for large changes]

ICLR23Paper: Make sure to reference. First time the holo calc idea was introduced (afaik). But(!): only for functions decaying at infinity AND used different definition. How explicit of a comparison to include?

Contrary to spatial convolutions, spectral convolutions are shown to be able to capture inherent geometric
%intrinsic 
notions of stability 
%\textcolor{red}{(limits?)} of directed graphs and provide new state of the art results on a wide selection heterophilic node-classification benchmarks.
[Need to emphasize that others have used the "functions of operators idea" on graphs. also check levies exact formulatiopn]
Characteristic operator: derivative is generator of translations, for us we need to choose the right operator also on graphs: (\textbf{not only the Laplacian})
Jordan Chevalley theory
interplay of correct functions with correct operators
check how WLgoTOP referenced previous work

ICLR23 looked at it from a stability perspective

do CORA, Pubmed, Citeseer MS-Acad!!!!!!!!!!!!!!!!!!!!!!!!


it has recantly been mentioned that directedness improves accuracy on heterophilic graphs. We are even better

Nilpotent matrix not diagonaliable (https://math.stackexchange.com/questions/1820350/any-nilpotent-matrix-is-not-diagonalizable)

Basis in which stuff is learned and inductive bias to drop zero order. (heterophily) How to interpret in a spectral manner?


Issues of multiplicity sweeped under rug

Ruiz graphon also graph Fourier trafo https://arxiv.org/pdf/2006.03548.pdf



